WinoCNN: Kernel Sharing Winograd Systolic Array for Efficient Convolutional Neural Network Acceleration on FPGAs

The combination of Winograd's algorithm and systolic array architecture has demonstrated the capability of improving DSP efficiency in accelerating convolutional neural networks (CNNs) on FPGA platforms. However, handling arbitrary convolution kernel sizes in FPGA-based Winograd processing elements and supporting efficient data access remain underexplored. In this work, we are the first to propose an optimized Winograd processing element (WinoPE), which can naturally support multiple convolution kernel sizes with the same amount of computing resources and maintains high runtime DSP efficiency. Using the proposed WinoPE, we construct a highly efficient systolic array accelerator, termed WinoCNN. We also propose a dedicated memory subsystem to optimize the data access. Based on the accelerator architecture, we build accurate resource and performance modeling to explore optimal accelerator configurations under different resource constraints. We implement our proposed accelerator on multiple FPGAs, which outperforms the state-of-the-art designs in terms of both throughput and DSP efficiency. Our implementation achieves DSP efficiency up to 1.33 GOPS/DSP and throughput up to 3.1 TOPS with the Xilinx ZCU102 FPGA. These are 29.1\% and 20.0\% better than the best solutions reported previously, respectively.

==> bak/sec3.tex <==


\section{Problems and Solutions}\label{sec:moti}

Most of the existing designs adopt $F(2\times 2,3\times 3)$ Winograd's algorithm as the basic Winograd acceleration unit, which is originally designed for accelerating the $3\times 3$ convolution layers \cite{8839351, sparsewino}. 
However, in latest DNNs such as ResNet~\cite{resnet}, GoogleNet \cite{qiu2016going}, Mobilenet \cite{howard2017mobilenets} and NasNet \cite{zoph2018learning}, $1\times1$ convolution becomes a common feature with remarkable model size reduction.
Meanwhile, the prevailing DNN quantization and low precision techniques~\cite{ul2q, vecq} increase the potential of boosting the hardware implementation performance, which, however, is not well explored by the existing Winograd-based convolution accelerators. For instance, most Winograd-based accelerators either process floating point data type or require large data-width, e.g., 16 bits.
In this section, we analyze the above mentioned design challenges, aiming to solve these two problems effectively.

\todo[inline]{
The novelties of our paper: \\
1. sharing \\
2. flexibility: supporting multi-level configurations \\
3. system integration
}


\subsection{Design Challenges}
{
In most hardware implementation of Winograd convolutions, the size of convolution kernel $g$ is fixed. 
To provide a new and flexible solution in dealing with convolution layers with other convolution kernel sizes, we may split the original large convolution kernel into smaller convolution kernels that fit for the adopted Winograd convolution configurations. 
For example, to compute a $7\times7$ convolution layer with $F(2\times2,3\times3)$ Winograd convolution, we may split the $7\times7$ convolution kernel into nine $3\times3$ convolution kernels with {unaligned kernel elements set to zero}.  
This way a single Winograd convolution PE can deal with convolution layers with different convolution kernels. We then analyze the ideal DSP efficiency of a Winograd-based accelerator with different Winograd convolution kernels (including $F(4\times4,1\times1)$, $F(2\times2,3\times3)$, $F(4\times4,3\times3)$ and $F(2\times2,5\times5)$ ) for different convolution kernel sizes ranging from $1\times1$ to $9\times9$, to show the critical challenges of {producing} resource-efficient and computation-efficient accelerator designs. 
Here, we define the DSP efficiency as the effective computation throughput in the unit of GOP/s provided by per DSP slice.
We set the system frequency of the accelerator as 200 Mhz and all the element-wise multiplication operations in the Winograd convolution are performed by on-chip DSPs with no idle cycles. 
We also estimate a potential double pumping (DP) technique for the accelerator, where the DSPs are driven by clocks with twice the frequency as the system clock.
The evaluation results are shown in Figure \ref{fig:perf_eff_comp} and are used as a guideline to choose proper Winograd convolution configurations in our implementation.}





% There are three critical challenges that are observed from the baseline evaluations.

% \red{Use one paragraph to explain the figure}



%  We evaluate the ideal effective DSP efficiency of different Winograd Processing Elements (PEs) with different Winograd convolution configurations including $F(4\times4,1\times1)$, $F(2\times2,3\times3)$, $F(4\times4,3\times3)$ and $F(2\times2,5\times5)$ under 200 Mhz working frequency when dealing with convolution layers with different convolution kernel .  We assume that the when the convolution kernel size is larger than the Winograd convolution kernel size, the convolution is complete by splitting the original convolution into smaller convolution kernels. 

\begin{figure}[h]
  \centering
  \vspace{-10pt}
%   \includegraphics[width=0.4\textwidth]{figures/wino_effi.png}
  \includegraphics[width=0.48\textwidth]{figures/figure1-crop.pdf}
  \vspace{-12pt}
  \caption{DSP efficiency of different Winograd filters on different convolution kernel sizes.}
  \label{fig:perf_eff_comp}
  \vspace{-12pt}
\end{figure}




\subsubsection{Flexibility of Winograd convolution}

\red{The constant transformation metrics of the {Winograd} algorithm results in the difficulty of reusing the \textbf{acceleration pattern} among different kernel sizes.}
% challenge of designing a PE with flexible support for different kernel sizes.
% As shown in Figure~\ref{fig:perf_eff_comp},
Conventionally, to compute $1\times1$ convolution, traditional implementation of Winograd algorithms need to expand $1 \times 1$ convolution to  $3 \times 3$ or instantiate
dedicated accelerators/logic for $1\times 1$ convolution only, which will result in significant waste and inefficient resource utilization. As can be seen with the {red line in Figure~\ref{fig:perf_eff_comp}}, the DSP efficiency of executing $1 \times 1$ convolution using $F(2\times2, 3\times3)$ accelerator is only $\frac{1}{9}$ of the DSP efficiency of executing $3\times3$ convolution.
Hence, designing a {Winograd-based} PE with flexible support for different kernel sizes while maintaining high DSP efficiency is essential but remain unexplored. 
However, upon the exploration of Winograd convolution algorithm, we observe that there is good potential for performance improvement while sharing of DSP resource among different Winograd convolution kernels, i.e., using the same set of DSPs to compute $F(4\times4, 1\times1)$ and $F(2\times2, 3\times3)$ could easily obtain the high performance for different convolution kernel sizes.
We could also easily obtain the ideal DSP efficiency of 2 sets of Winograd convolutions sharing DSP resources.
% , in Figure. \ref{fig:perf_eff_comp} in dotted lines. 
The achievable DSP efficiency for {Winograd} based convolution is shown as the green dotted line in Figure~\ref{fig:perf_eff_comp}, when DSPs are shared between $F(2\times2, 3\times3)$ and $F(4\times4, 1\times1)$ with the DSP double pumping techniques.
The details of resource sharing between Winograd convolutions will be further discussed in Section \ref{sec:sharing}.


% \subsection{Precision Requirement in Practices}

% For an FPGA implementation, the computational precision becomes a practical consideration of the design.
% For the $6 \time 6$ filter based Winograd implementation, there requires an addition 7 bits during the execution of the transformation matrix to maintain the precision of the accuracy. However, this further leads to an under utilization of the DSP resource by hindering the use of DSP double-pumping or even DSP double-splitting to take advantage of the given DSP resources.
% Even for the models with lower bitwidth training, e.g. 4bits quantization, the intermediate results requires 11 bits to be executed precisely.
% However, this situation is naturally solved by the smaller kernel sizes, which has a less effect on the precision of the transformation. e.g., wino4x4 only requires 5 additional bits to maintain the original accuracy. The lower bitwidth requirement for the execution enables the design to take advantage of the DSPs and further boost the performance of the Winograd-based convolution acceleration. As shown in the Figure.~\ref{}, with wino4x4, the DSP double-pumping and DSP double-splitting further boosts the DSP efficiency to a state-of-the-art value.


\subsubsection{Efficiency and precision trade-off}

The Winograd algorithm reduces the number of multiplications in the convolution, and the reduction ratio varies with the Winograd convolution configurations.
In Table \ref{tab:multi_redu}, we list the reduction ratio of Winograd convolution with different Winograd filter configurations.
Ideally, a larger Winograd input tile size leads to a higher multiplication reduction rate.


\begin{table}[h]
    \centering
    \vspace{-6pt}
    \caption{Multiplication reduction ratio of different Winograd tile {sizes} for different convolution Kernels}
    \vspace{-6pt}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \hline
        & F(4x4,1x1) & F(2x2,3x3) & F(4x4,3x3) & F(2x2,5x5)  \\ \hline
        Tile size & 4 & 4 & 6 & 6 \\ \hline
        Ratio & 1 & 2.25 & 4  & 2.78  \\ \hline
        \hline
    \end{tabular}
    \label{tab:multi_redu}
    \vspace{-6pt}
\end{table}



On the other hand, 
the computational precision, i.e., the bit-width, is an important factor for hardware implementation.
Since the Winograd transformation involves bit-shift and adding operations, it requires larger data bit-width for the transformation output to prevent data overflow.
For the Winograd convolution configuration $F(4\times4,3\times3)$ and $F(2\times2,5\times5)$, maintaining the computation accuracy requires additional 10 bits during the execution of the weight transformation, which may resulting transformed weight data exceeding 16 bits. 
This will result in an under utilization of the DSP resource by hindering DSP double-pumping which is a promising technique that can double the DSP efficiency, since the DSP double pumping only supports 16 bits multiplications in HLS.
This problem can be naturally resolved by using smaller Winograd convolution configurations, {which has less effect on the required data bitwidth in the transformation.} {For example}, $F(4\times4,1\times1)$ and  $F(2\times2,3\times3)$ Winograd convolution only {requires} 4 additional bits during the matrices transformation to maintain the data accuracy. The lower bitwidth requirement for the execution enables the design to take advantage of the DSPs and further boost the performance of the Winograd-based convolution acceleration with advanced DSP technologies for lower bitwidth processing. As shown in Table~\ref{tab:bit_increment}, only with the $F(4\times4,1\times1)$ and  $F(2\times2,3\times3)$  Winograd configurations, the DSP double-pumping can be enabled to boost the DSP.


\begin{table}[h]
    \centering
    \vspace{-6pt}
    \caption{Change of minimum data bitwidth after Winograd transformation}
    \vspace{-6pt}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \hline
        &F(4x4,1x1) & F(2x2,3x3) & F(4x4,3x3) & F(2x2,5x5)  \\ \hline
        Weight & +2 & +4 & +8  & +8  \\ \hline
        Input  & +4 & +4 & +10 & +10 \\ \hline
        \hline
    \end{tabular}
    \label{tab:bit_increment}
    \vspace{-12pt}
\end{table}



% \begin{table}[h]
%     \centering
%     \caption{Bit increment in different Winograd Kernels}
%     \vspace{-6pt}
%     \begin{tabular}{c|c|c|c}
%         \hline
%         \hline
%          wino-filter size     & 1x1 & 3x3 & 5x5  \\ \hline
%         4x4: input  & 4   & 4   & N/A  \\ \hline
%         4x4: weight & 2   & 4   & N/A  \\ \hline
%         6x6: input  & 8   & 8   & 8  \\ \hline
%         6x6: weight & 10  & 10  & 10  \\ \hline
%         \hline
%     \end{tabular}
%     \label{tab:bit_increment}
%     \vspace{-10pt}
% \end{table}


\subsubsection{Data access requirement}
Recent designs of systolic arrays for CNNs involve sizable external data access,
while the Winograd convolution requires access of input tile data from input feature-maps. 
Both requirements increase the intensity and complexity of data access, which would introduce a memory bottleneck and degrade the overall performance. 


\subsection{Our Proposed Solutions}
Based on the above analysis, we propose our WinoCNN accelerator system that specifically address the three critical design challenges:
\begin{itemize}
    \item For the efficiency of the PEs, we propose a \textbf{resource sharing Winograd convolution based processing element (WinoPE)} that could flexibly support different kernel sizes without additional resource requirement.
    \item For the effectiveness of the data access, we propose an \textbf{efficient memory sub-system that supports the planar data access with pipelined PEs} to dramatically improve the data access.
    \item For the accelerator system, we propose a \textbf{configurable systolic array architecture with WinoPEs (WinoCNN)}, and further improve its flexibility by accurate modeling of the resource and performance of it.
\end{itemize}

% The novel designs above improve the dynamic utilization of the computing resources for our target FPGA platform. 
The detailed design principle for each component will be presented in the following section.


==> bak/sec5.tex <==
\section{WinoPE: PE with kernel sharing} \label{sect:wino_conv}

\todo[inline]{Is it possible to merge the WinoPE design, mem-system and systolic array construction into a single section, and title it as implementation?
I feel we have reasoned the design concepts in the previous section quite clear, what should follow it is just the design.
The mem-system we have is not only for the PE, but also serves the systolic array architecture, so it should come after the PE and systolic array.}

% In this section we introduce the detailed technologies for our proposed WinoCNN PE, especially the design of reusing the same PE for different convolution kernel sizes without resource overhead.
Our Winograd processing elements (WinoPE) is the basic computation unit of the Winograd systolic convolution accelerator system (WinoCNN), where each PE is able to complete the computation in Eq.~\ref{eq:otrans} with an initiation interval (II) of a single clock cycle.
Our WinoPE is featured with the flexible support for different convolution kernel sizes without resource overhead. It adopts the most popular $F(4\times4, 1\times1)$ and $F(2\times2, 3\times3)$ Winograd computations and processes them with a unified architecture.
Figure \ref{fig:wino_cell} shows the architecture of one WinoPE.
A WinoPE contains an input tile register (red block), a weight tile register (blue block), a matrix of multipliers (purple circle), an output transformation module (green block), and an output tile (light yellow block for ($4\times4, 1\times1$) and dark yellow block for ($2\times2, 3\times3$)) towards an output buffer.

\begin{figure}[h]
    \centering
    \vspace{-6pt}
    \includegraphics[width=0.43\textwidth]{figures/winocell.png}
    \vspace{-10pt}
    \caption{WinoCNN processing element.}
    \label{fig:wino_cell}
    \vspace{-10pt}
    
\end{figure}

Based on Eq.~\ref{eq:itrans} to Eq.~\ref{eq:otrans}, in each working cycle, the PE first reads a tile of input data and a tile of weights.
Note that all the elements of input data and weights need to be read in parallel; it requires special technologies for simultaneous planar data access, which will be discussed in Section~\ref{sect:data_opt} in detail.
After fetching the input/weight data, the multiplier matrix performs element-wise multiplication as in Eq.~\ref{eq:eltmul}, and outputs the result of $U\odot V$. 
The output transformation module takes the results of $U \odot V$ and computes Eq.~\ref{eq:otrans}.

As discussed in Section 3, for different Winograd convolutions $F_1(m_1 \times m_1, r_1 \times r_1)$ and $F_2(m_2 \times m_2, r_2 \times r_2)$, as long as $m_1 + r_1 - 1 = m_2 + r_2 - 1$, the sizes of $U_1$ and $V_1$ are equal.
Therefore, the data reading and the element-wise multiplication modules can be reused.
After obtaining matrix $U \odot V$, since the size of transformation matrix $A^T$ varies for different kernel sizes, the following computation cannot be directly 
reused.
To solve this problem for the adopted $F(4\times4, 1\times1)$ and $F(2\times2, 3\times3)$ Winograd algorithms, we propose a selectable output transformation matrix $A^T_{sel}$, in which we insert a \textbf{selection bit} $sel$ into the matrix $A$ as the follow:
\begin{equation}
\begin{small}
A^T_{sel} =  \begin{bmatrix}
    1 & 1 & 1 &  0\\
    0 & 1 & -1& -\textbf{sel}\\
    0 & 1 & 1 &   0\\
    0 & 1 & -1  & 1
   \end{bmatrix}
\label{eq:select_out_trans}
\end{small}
\end{equation}
When $sel$ is set to 0, the PE performs $F(4\times 4,1\times 1)$ algorithm, where the whole $4\times 4$ matrix is the output of the Winograd algorithm $Y$. When $sel$ is set to 1, the PE performs $F(2\times 2,3\times 3)$ algorithm, where the top left four elements of the result matrix is the Winograd output $Y$.
In this way, the whole PE can be reused by different kernel sizes of Winograd with no DSP overhead.
Finally, the computed outputs are stored in the output buffer constructed with BRAMs.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/winocell_vect.jpg}
%     \caption{Winograd Convolution Processing Element}
%     \label{fig:wino_cell_vect}
% \end{figure}

Furthermore, we partition the input tile register $U$ and weight tile register $V$ into individual registers that each contains a single data from the input channels, so that the multiplication for the entire tile could be finished in a single clock cycle. 
An adder tree inside the $U\odot V$ module accumulates the multiplication results along the channel dimension.

Due to the restriction of logical delay and routing issues, modern FPGA applications usually have a typical working frequency from 100MHz to 300Mhz. 
However, the DSP slices are designed to work at a much higher clock frequency. A DSP48E2 slice on a Xilinx Ultrascale architecture (eg. Zync Ultrascale+ 102) can achieve 600Mhz. 
Several previous work have discussed about DSP multi-pumping and demonstrated that it greatly increases DSP efficiency~\cite{6513499}. 
In our design, We drive the DSP with $2\times$ system frequency and thus double the DSP efficiency. The double pumping DSP is able to compute the sum of two product in one system clock cycle. 
% Then a LUT based adder tree is following it and conducts the sum up of the output from the DSPs.

==> bak/sec6.tex <==
\section{Memory sub-system} \label{sect:data_opt}

% The computation pattern of Winograd requires planar data access in parallel, which brings in a challenge for efficient memory control and data fetching for the PEs.
% As the example shown in Fig.~\ref{fig:loc_map}, 
% for the first PE, it requires 16 data simultaneously (circled by red) with indices $(x, y)$ where $x \in [1, 4]$ and $y\in [3, 6]$;
% for the second PE, it requires another 16 data simultaneously (circled by blue) with indices $(x, y)$ where $x \in [1, 4]$ and $y\in [5, 8]$.
% They also share two columns of data (circled by pink).
% For an efficient PE design,
% first, the data must be fetched in parallel;
% second, the overlapped data shall be reused.
 

As is discussed in Section~\ref{sec:sharing}, to access the data (including weights and feature-maps) efficiently, according to our design principles,
we propose:
(1) a BRAM buffer matrix that has a unique addressing mechanism to support efficient parallel data access, and (2) a pipelined planar data control and organization for our WinoPEs.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/tile_access.png}
    \vspace{-6pt}
    \caption{Input tile planar access}
    \label{fig:tile_access}
    \vspace{-15pt}
\end{figure}
% \vspace{-6pt}

\subsection{BRAM Buffer Matrix}

To guarantee the parallel access of the input tiles, we fold the input feature-maps into a matrix of BRAM buffers, 
denoted as $BRAM_{in}[H_b][W_b][D_b]$, which consists of $H_b \times W_b$ BRAM buffer instances (or BRAM bank) of depth $D_b$, as shown in Figure~\ref{fig:tile_access}. 
Each BRAM buffer instance has its independent address port and data port, hence total $H_b \times W_b$ data can be accessed from the BRAM buffer matrix each cycle at different addresses.
An address mapping mechanism is designed as shown in Eq.~\ref{eq:bram_map} to decide the location in the buffer $BRAM_{in}[h][w][addr]$ for a certain input pixel in the feature map $in[id][r][c]$, where $ID,id,r,c$ represent the input feature map depth, depth index, row index and column index for the pixel:
\begin{equation}\label{eq:bram_map}
\begin{gathered}
h=r \% H_b, ~
w=c \% W_b\\
addr = concat(\left \lfloor{\frac{r}{H_b}}  \right \rfloor, \left \lfloor{\frac{c}{W_b}} \right\rfloor\cdot ID+id )\\ 
\end{gathered}
\end{equation}

Meanwhile, we implement an address matrix to store the addresses of the BRAM banks in the BRAM matrix.
The address of the BRAM bank is the concatenation of high and low address bits as shown in Eq.~\ref{eq:bram_map}. 
The high address bits are computed by $\left \lfloor{\frac{r}{H_b}} \right\rfloor$ and low address bits are computed by $\left \lfloor{\frac{c}{W_b}} \right\rfloor\cdot ID+id$.
The BRAM banks in the same row share the same high address bits, while the BRAM banks in the same column share the same low address bits.

\begin{figure}[h]
    \centering 
    \includegraphics[width=0.40\textwidth]{figures/firststage_revise.png}
    \vspace{-6pt}
    \caption{Data addressing in BRAM}
    \label{fig:loc_map}
    \vspace{-6pt}
\end{figure}

As an example, we assume $H_b = 4, W_b = 8, W = 4, K = 2$ and $N = 2$ and we need to access two input wino tiles $in[0][1\text{:}4][3\text{:}6]$ and $in[0][1\text{:}4][5\text{:}8]$, enclosed by red and blue circle in Figure \ref{fig:loc_map}, in parallel. The union of the two input wino tiles can be represented as $in[0][1\text{:}4][3\text{:}8]$. 
According to the address mapping defined in Eq.~\ref{eq:bram_map}, the pixels in the $in[0][1\text{:}4][3\text{:}8]$ are accessed from four different regions of BRAM buffer matrix with different high address bits and low address bits as shown in Figure \ref{fig:loc_map}. 
By configuring the high address bits and low address bits in the address matrix, we can access all the data in $in[0][1\text{:}4][3\text{:}8]$ from the BRAM matrix simultaneously in one clock cycle.

\subsection{Planar Data Access}

We represent the sequence of input Winograd tiles as $T_N$, where $T_N$ consists of $N$ tiles with $[W,W]$ size that are defined as
\begin{equation}
T_N[n]=
in[id][ri\text{:}ri\text{+}W\text{-}1][ci\text{+}nK\text{:}ci\text{+}nK\text{:}\text{+}W\text{-}1] 
\end{equation}

All the elements in $T_N$ forms an continuous input data block, denoted as $T_U$, with size $[W, (N\text{-}1)K\text{+}W]$:
\begin{equation} \label{eq:inplane_blk}
\begin{gathered}
T_U=\bigcup_{n\text{=}1}^{N-1}T_N[i]=
in[id][ri\text{:}ri\text{+}W\text{-}1][ci\text{:}ci\text{+} (N\text{-}1)K\text{+}W\text{-}1] 
\end{gathered}
\end{equation}

The input tiles required by the WinoPEs are fetched from the BRAM matrix system in a 3-stage pipeline,
% In the first stage all the data required for one PE row are fetched from the BRAM matrix. In the second and third stage, the fetched data are reorganized in row-wise and column-wise respectively through the mux arrays between stage register matrices. 
% The BRAM matrix system also includes three pipelined stage  of register matrix 
as shown in Figure \ref{fig:pipestage}. 
The first stage of register matrix (denoted as \textit{plane tile}) is of size $H_b \times W_b$ and is directly connected to the data port of the BRAM matrix. 
The second stage of register matrix (denoted as \textit{row plane tile}) is connected with the \textit{plane tile} through a multiplexer array so that each row of the \textit{row plane tile} can be selected and loaded from one arbitrary row of the \textit{plane tile} to the row plane tile. 
The third stage of register matrix (denoted as \textit{input wino tiles} ) is connected with \textit{row plane tile} through a multiplexer array with column selection.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/threestagearchi.png}
    \vspace{-6pt}
    \caption{Pipeline stages of input data system}
    \label{fig:pipestage}
    \vspace{-12pt}
\end{figure}

Eventually, with our BRAM buffer matrix and Planar data access and reorganization control, the input feature-maps are reorganized as data tiles and provided to each of the WinoPE in our system.



\subsection{Other Buffers}
% The memory sub-system also contains the weight buffer and output buffer. The output buffer is design as a a ping-pong buffer that constructed with 2 individual buffers to eliminate the long write latency to external memory.

The PE array requires continuous weight data streaming from the input interfaces. However, the PE array may request same weight data multiple times. 
To take advantage of the DDR burst performance and the support of random access of the on-chip BRAMs, 
we fetch the weight data from DDR with a continuous and address-consecutive manner and store them in the on-chip buffers constructed with BRAMs, and then access the weight data from the buffers to avoid multiple external memory access for the same weight data.
% we prefer a continuous and address-consecutive data access pattern from DDR for the off-chip weight loading process. To achieve data access continuity and consecutively while avoiding multiple loading of the same data from DDR, we construct the weight buffer with BRAMs then read the weight data from them with random access pattern and provide the read out to the PE array.}
% Figure \ref{fig:weightfeed} illustrates the architecture of the weight data system.  The system contains $M$ weight BRAM buffers with each BRAM buffer corresponding to one row in the PE array. 
% In our implementation, we store the weight data with the expected accessing order in off-chip memory so that the weight data can be load consecutively into the on-chip BRAM buffer. 
The BRAM buffers have the same data width as the total data width of the weight tile in the PE.
The output buffer is designed as a ping-pong buffer to reduce the write back latency to external memory.




==> bak/sec7.tex <==
% \section{WinoCNN Architecture Detail}\label{sec:archdetail}


% We demonstrate our WinoCNN design in this section. In section \ref{sect:over_arch} we present the overall architecture and module scheduling of our convolution accelerator. In section \ref{sect:wino_conv} we illustrates a scalable Winograd systolic convolution system that enables parallel execution of Winograd algorithm. The architecture of the data system which resolves the data stream requirement for the  Winograd systolic convolution system is presented in section \ref{sect:data_opt}.


\section{WinoCNN accelerator system} \label{sect:over_arch}

Our WinoCNN accelerator system contains both the accelerator system architecture for FPGA implementation and the software libraries that are executable on the processor.

\subsection{WinoCNN Architecture Overview} \label{sec:winocnn_system}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/architecture.png}
    \caption{Overall architecture}
    \label{fig:architect}
    % \vspace{-12pt}
\end{figure}


The overall architecture of our proposed WinoCNN accelerator system is shown in Fig.~ \ref{fig:architect}.
It includes the memory subsystem and the systolic array constructed with our WinoPEs.
% our core modules for efficient data access (blue block) and Wino-PEs as a systolic array for parallel Winograd computation (yellow block). as well as input buffers, output buffers and off-chip DDR memory.
% The systolic PE array is composed of our proposed Wino-PEs, which is able to handle flexible Winograd kernel sizes.
Note here, the flexible kernel size support is provided by our WinoPEs.
% The input buffers are dual-port line buffers which are capable of simultaneous data reading and writing.
% The output buffers are ping-pong buffers.
% \textcolor{blue}{The WinoCNN PE design will be introduced in Section \ref{sect:wino_conv}, and the systolic array system will be introduced in Section \ref{sec:winocnn_system}. The planar data access block is the memory management system we proposed, which enables parallel data access for the unique computation pattern of WinoCNN PEs and to be introduced in Section \ref{sect:data_opt}.}
The convolution layers of the input models are computed in output row stationary. Each time a fixed number of output rows are computed. The input reading, computation, and output data offloading are scheduled to run simultaneously.
Algorithm 1 demonstrates the overall execution flow. 
The convolution is divided into several sub-procedures with each sub-procedure computing $RS$ rows of the output feature-map. 
An input reading process first loads required input data from off-chip memory into the on-chip BRAM buffers (line \ref{line:read_input_first}). Then a loop computes the required output tiles consecutively (line 7 to 15). 
Each iteration in the loop includes three processes: read-input process (line 8), computation process (line 10), and write-output process (line 12). 
The read-input process loads input data for computation required by the next iteration into the input BRAM buffer. The computation process computes the output tile with the data from input BRAM buffer and weights from off-chip memory, then store the result into one of the output ping-pong buffers. The write-output process writes the outputs computed in the previous iteration to external memory. 
% As shown in Table \ref{tab:port_occupation}, 
With the scheduling above and dual port provided by the BRAMs, no port conflict exists among the three processes and the three processes executes simultaneously.

\begin{algorithm}
\caption{Convolution schedule on WinoCNN}\label{euclid}
\footnotesize
\begin{algorithmic}[1]
\Procedure{Conv}{$\textbf{Ports}:in,out,weight$}
\State $BRAM_{in}, BRAM_{out,2} $
\State $r_i=\text{-} P, r_c=0, r_o=\text{-} RS$
\State $p=0$
\State $BRAM_{in} \gets in[r_i,r_i+RS+K-1]$ \label{line:read_input_first}
\State $r_i=r_i+RS+K$
\While{$r_c < OH$}
\State $BRAM_{in} \gets in[r_i,r_i+RS-1] $ \label{line:read_input}
\State $r_i=r_i+RS$
\State $comp(BRAM_{in}, w, BRAM_{out,p}, r_c, r_c+RS-1)$\label{line:compute}
\State $r_c=r_c+RS$
\State $out[r_o,r_o+RS-1] \gets BRAM_{out,1-p} $ \label{line:write_output}
\State $r_o=r_o+RS$ 
\State $p=1-p$
\EndWhile
\State $out[r_o,r_o+RS-1] \gets BRAM_{out,1-p} $
\EndProcedure
\end{algorithmic}
\label{alg:conv_schedule}
\end{algorithm}

% \begin{table}[h]
%     \centering
%     \renewcommand{\arraystretch}{0.9}
%     \small
%     \caption{Memory Port Occupation}
%     \label{tab:port_occupation}
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{c|c|c }
%     \hline
%     \hline
%     Process &  BRAM port & DDR port \\\hline
%     Read-Input & $BRAM_{in}$:$write$ & in  \\ \hline
%     Computation & \begin{tabular}{c}$BRAM_{in}$:$read$\\ $BRAM_{out,p}$:$read$ \\$BRAM_{out,p}$:$write$\end{tabular} & weight\\ \hline
%     Write-output & $BRAM_{out,1-p}$:$read$&  out \\
%     \hline
%     \hline
%     \end{tabular}
% \end{table}



% Given the advantages of the systolic array architecture such as high parallelism and efficient data reuse, we organize our Winograd PEs systolic array architecture, forming a Winograd systolic convolution system, called WinoCNN, as shown in Figure \ref{fig:winosystolic}.
The WinoCNN system accepts the input tiles in a streaming manner from the top side and the corresponding weight data stream from the left side. The input data and the weights are registered in the WinoPE cell to form the internal systolic data transaction.


\subsection{WinoPE Systolic Array Construction}

% The Winograd systolic convolution system is constructed by arranging WinoPEs in $M\times N$ matrix. To accommodate the data and computation flow, 
Originally, the computation process in Algorithm \ref{alg:conv_schedule} is organized as the loop in Fig. \ref{lst:win_loop}. The symbol representations are specified in Table \ref{tab:sym_rep}. 
% In the listing, 
Loop \texttt{L0} iterates through the output depth with a step of $M$.
Loop \texttt{L1} segments the output row into {Winograd output tile} of size K.
Loop \texttt{L2} segments the output columns into N Winograd tiles.
Loop \texttt{L3} iterates through all the input depth.
In order to increase the parallelism of data processing,
generally the inner loop \texttt{L4} to \texttt{L5} is flattened as the $M\times N$ PE array which processes $N$ output tile across $M$ output depth each cycle. 
Easy to know, all the WinoPEs with same $m$ index share the same weights, and the WinoPEs with same $n$ index share the same input tile.
% The red square in Figure \ref{lst:win_loop} shows an example of behaviour and data flow in a flattened PE arrays with dimension $2\times2$.
% {Such data sharing makes it possible to construct a Wingrad systolic array.}


% \vspace{6pt}
\lstset{style=mystyle}
% \begin{lstlisting}[language=C++,caption=Loop for Computation Process,
% label={lst:win_loop},escapechar=|]
% ||
% \end{lstlisting}
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/winoflatten_code.png}
    \vspace{-6pt}
    \caption{Loops of computation process}
    \label{lst:win_loop}
    \vspace{-12pt}
\end{figure}


% an paragraph on how the PE work

% \textcolor{blue}{Xinheng: following paragraph may require polish}
However, the flattened array shares a single data and broadcast to all PEs in the same clock cycle which lead to high fanout and worse implementation timing. An example of $M\times N = 2\times2$ square is shown in the red square in Fig.~\ref{lst:win_loop}.
Instead, we construct the WinoPEs in $M\times N$ matrix as systolic array that shares the data by shifting the weight and input among WinoPEs that could well utilize the on-chip storage and reduce the high fanout issues for the implementation.
% of sharing the data through the broad casting in the flatten architecture, our systolic array architecture shares the data by shifting the weight data and input data among PEs.
In order to achieve this, we first re-design the PEs with FIFO interfaces (as shown in Fig.~\ref{lst:pe_loop}).
% and then reorganize the overall array as Fig. \ref{lst:pe_loop}.
Here, the loop \texttt{L0-L3} are the same as the one in Fig. \ref{lst:win_loop}; however, the input Winograd tile and the weight tile are fetched from the top and left FIFO interface which connects to the top and left neighbours of the PE respectively.
Meanwhile, in the same iteration, the input and weight data are pushed into bottom and right FIFO interface and passed to the bottom and right neighbours respectively. 
Due to the block mechanism of the FIFO, one PE has to wait for the data from its top neighbour and left neighbour. 
Therefore one PE is always one iteration delay off its top and left neighbour.
Also, since the input data are shared through the same column and the weight data are shared through the same row of the computation array, the input and weight data passed in by the top and left neighbours are exactly the required data for the current WinoPE. 

% The PEs are connected through FIFOs (stream instances in vivado HLS) to construct the systolic system. 
% Figure \ref{lst:pe_fifo} shows the pseudo code of construction of a $2\times2$ systolic architecture with FIFOs and PE modules.
% Eventually, our winoCNN system is constructed with the systolic array of WinoPEs as shown in the red square  Figure~\ref{lst:pe_fifo}.
With the modification of the FIFO interfaces designed for our WinoPEs, we could simple instantiate two FIFO arrays for the row connection and the column connection, denoted as $row\_fifo[M][N]$ and $col\_fifo[N][M]$ that could be used to organize the WinoPE systolic array. The $M, N$ parameters are configurable during the WinoCNN system generation.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/PE_loops.png}
    \vspace{-6pt}
    \caption{Loop behaviour for PE$_{m,n}$}
    \label{lst:pe_loop}
    \vspace{-12pt}
\end{figure}



% \lstset{style=mystyle}
% \begin{lstlisting}[language=C++,caption=Loop Behaviour for PE$_{m,n}$$,
% label={lst:pe_loop},escapechar=|]
% module_PE(
%     input FIFO: left_fifo, top_fifo
%     output FIFO: right_fifo, bottom_fifo)
% {
%     L0:for(od=0;od<OD;od+=M)
%     L1:for(r=r_c;r<r_c+RS;r+=K) 
%     L2:for(c=0;c<OW;c+=K*N)
%       ri=r-P; ci=c-P;
%     L3:for(id=0;id<ID;id++)
%     {
%         #pragma HLS pipeline
%         U=top_fifo.dequeue();
%         bottom_fifo.equeue(U);
%         //itrans(in[id][ri:ri+W-1][cn:cn+W-1]) 
%         V=left_fifo.dequeue();
%         right_fifo.equeue(V);
%         //wtrans(weight[id][od+m][:][:]);
%         Y=otrans(U*V)
%         oc=c+n*K;
%         if(id==0)
%             out[od+m][r:r+K-1][oc:oc+K-1]=Y;
%         else
%             out[od+m][r:r+K-1][oc:oc+K-1]+=Y;
%     }
% }

% \end{lstlisting}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/fifo_connect.png}
%     \caption{FIFO connection of PEs}
%     \label{lst:pe_fifo}
% \end{figure}




% \begin{lstlisting}[language=C++,caption=Loop Behaviour for PE$_{m,n}$$,
% label={lst:pe_fifo},escapechar=|]
% #pragma HLS dataflow
% hls::stream row_fifo[2][2]; // FIFOs between PEs at same row
% hls::stream col_fifo[2][2]; // FIFOs between PEs at same colum

% module_PE<0,0>(row_fifo[0][0],col_fifo[0][0],row_fifo[0][1], col_fifo[0][1])
% module_PE<0,1>(row_fifo[0][1],col_fifo[0][1],DUMMY, col_fifo[1][1])
% module_PE<1,0>(row_fifo[1][0],col_fifo[1][0],row_fifo[1][0], DUMMY)
% module_PE<0,1>(row_fifo[0][1],col_fifo[0][1],DUMMY, DUMMY)
% \end{lstlisting}


% an paragraph on how to write new code ?

\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{0.9}
    \footnotesize
    % \vspace{-5mm}
    \caption{Symbol Representation}
    \label{tab:sym_rep}
    \vspace{-6pt}
    \setlength{\tabcolsep}{2pt}
    \footnotesize
    \begin{tabular}{c|c}
    \hline
    \hline
    ID, IH, IW & \begin{tabular}{c}  The depth, height and width \\ of input feature-map \end{tabular}\\ \hline
    in[ID][IH][IW] & \begin{tabular}{c}  Input feature-map \end{tabular}\\ \hline
    OD, OH, OW & \begin{tabular}{c}  The depth, height and width \\ of out feature-map \end{tabular}\\ \hline
    out[OD][OH][OW] & \begin{tabular}{c}  Output feature-map \end{tabular}\\ \hline
    F & \begin{tabular}{c}  Convolution weight kernel size \end{tabular}\\ \hline
    weight[ID][OD][F][F] & \begin{tabular}{c}  Convolution weight \end{tabular}\\ \hline
    RS & \begin{tabular}{c} The  \# of rows processed in each iteration  \end{tabular}\\ \hline
    $r\_c/r_c$ & \begin{tabular}{c} The index of the first row processed \\ in each iteration  \end{tabular}\\ \hline
    W & \begin{tabular}{c} The size of Winograd input tile \end{tabular}\\ \hline
    K & \begin{tabular}{c} The size of Winograd output tile \end{tabular}\\ \hline
    M & \begin{tabular}{c} The height of Winograd systolic array \end{tabular}\\ \hline
    N & \begin{tabular}{c} The width of Winograd systolic array \end{tabular}\\ \hline
    Q & \begin{tabular}{c} The register vector size in PE \end{tabular}\\ \hline
    \hline
    \end{tabular} 
    \vspace{-12pt}
\end{table}



% \todo[inline]{Two questions for the red words above: 1. I am not sure if putting them here is proper. We should explain at the beginning of section 6 about the architecture of the systolic array. 2. It seems not quite important. Because if we use the Figure 6(a) organization, then it is actually not a systolic array.}

% \textcolor{blue}{Xinheng: What I want to express here is the which computation happens in which cell. I think there should be a better way to express the mechanism of the systolic array}
% \todo[inline]{I think we could add in a subsection about the configurable systolic array, which is an important point in our design and also been mentioned in the following modeling part.}



% \begin{figure}[h]
% \begin{subfigure}[b]{0.43\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/winoflatten.jpg}  
%      \caption{Flattened 4x4 PE array}
%  \label{fig:winoflatten}
% \end{subfigure}\\
% \begin{subfigure}[b]{0.43\textwidth}
%   \centering
%     \includegraphics[width=1\textwidth]{figures/winosystolic.jpg}
%     \caption{Systolic 4x4 PE array}
%     \label{fig:winosystolic}
% \end{subfigure}
% % \vspace{-4mm}
% \caption{PE arrays \textcolor{red}{Yao: I think using only 2 PEs for each figure is enough to show the idea, can we reduce the number of the PEs and merge them into the size of a single current figure?}}
% \label{fig:fig}
% \end{figure}
% \vspace{-18pt}


% \iffalse
% \subsubsection{Weight Data System}~\label{sect:weight_data_system}\\

% The PE array system requires continuous weight data streaming from the left side. However, from the analysis of the loop in Figure \ref{lst:win_loop}, the weight data is purely independent of index \texttt{r} and \texttt{c} in loop \texttt{L2} and \texttt{L3}, which means that the  PE array may request same weight data multiple times. Meanwhile, to make the most advantage of DDR burst mode, we prefer a continuous and address-consecutive data access pattern from DDR for the off-chip weight loading process. To achieve data access continuity and consecutively while avoiding multiple loading of the same data from DDR, we adopt the method of loading data consecutively into local BRAM then read the weight data from local BRAM with random access pattern. 
% Figure \ref{fig:weightfeed} illustrates the architecture of the weight data system.  The system contains $M$ weight BRAM buffers with each BRAM buffer corresponding to one row in the PE array. 
% In our implementation, we store the weight data with the expected accessing order in off-chip memory so that the weight data can be load consecutively into the on-chip BRAM buffer. 
% The BRAM buffer has the same data width as the total data width of the weight tile in the PE.
% The weight load module connects one weight DDR port with multiple BRAM buffers through the BRAM write port and can loads a tile of weight data consecutively from DDR port into the weight BRAM buffers connected to it with DDR burst in every single run.
% For the design with multiple DDR ports available for weight loading, the weight BRAM buffers are evenly allocated to all the DDR ports. 
% The feed module connects one BRAM buffer with one FIFO interface through the BRAM read port. It reads and streams the data from the BRAM with a pre-design pattern in every single run.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.40\textwidth]{figures/weightfeed.jpg}
%     \caption{Weigth Data System Structure}
%     \label{fig:weightfeed}
%     \vspace{-12pt}
% \end{figure}




% Then we schedule the runs of weight load module and feed module with a procedure illustrated in Algorithm \ref{alg:weightfeed_schedule}.
% We first partition address space of the BRAM buffer into two equal half, with each half serving one purpose between loading and reading data at one weight loading run or feed run. Then We segment the convolution weight in input depth and output depth dimension with tile size $T_i$ and $T_o$ respectively to accommodate the capacity of weight buffer. Accordingly, we reform the loop \texttt{L0} and \texttt{L1} in Figure \ref{lst:win_loop} into loop \texttt{L0\_0},\texttt{L1\_0}, \texttt{L0\_1}, and \texttt{L1\_1} as shown in Figure \ref{lst:win_loop_reform}. Within loop \texttt{L1\_0}, the computation process should only require data of weight tile $weight[idd\text{:}idd\text{+}T_i\text{-}1][odd\text{:}odd\text{+}T_oM\text{-}1] $.
% \begin{lstlisting}[language=C++,caption=Reformed Loop for Computation Process,label={lst:win_loop_reform},escapechar=|]
% L0_0:for(odd=0;odd<OD;odd+=M*T_o)
% L1_0:for(idd=0;idd<ID;idd+=T_i)
% L0_1:for(od=odd;od<od+T_o*M;od+=M) 
% L1_1:for(id=idd;id<id+T_i;id++)
% L2: ... ... ...
% \end{lstlisting}

% \begin{algorithm}
% \caption{Weight Streaming Schedule}
% \begin{algorithmic}[1]
% \Procedure{WeightFeed}{$weight, stream_M$}
% \State $BRAM_{w,M}$ 
% \State $odd_{p},idd_{p}$
% \For{$odd$ in $[0:MT_o:OD]$} \label{line:seg_od_loop}
% \For{$idd$ in $[0:T_i:ID]$} \label{line:seg_id_loop}
% \State $BRAM_{w,M} \gets weight[idd\text{:}idd \text{+}T_i\text{-}1][odd\text{:}odd$ $\text{+}MT_o\text{-}1]$
% \If{$odd \neq 0$ or $idd \neq 0$}
% \State $feed(BRAM_{w,0},stream_0,odd_{p},idd_{p})$
% \State $feed(BRAM_{w,1},stream_1,odd_{p},idd_{p})$
% \State $...$
% \State $feed(BRAM_{w,M-1},stream_{M-1},odd_{p},idd_{p})$
% \EndIf
% \State $odd_{p}=odd,idd_{p}=idd$ \label{line:write_output}
% \EndFor
% \EndFor
% \State $feed(BRAM_{w,0},stream_0,od_{p},id_{p})$
% \State $feed(BRAM_{w,1},stream_1,od_{p},id_{p})$
% \State $...$
% \State $feed(BRAM_{w,M-1},stream_{M-1},od_{p},id_{p})$
% \EndProcedure
% \end{algorithmic}
% \label{alg:weightfeed_schedule}
% \end{algorithm}


% The weight feeding procedure arranges a loop to load and stream all the weight tile in the order indicated in \texttt{L0\_0} and \texttt{L1\_0}. Each iteration in the loop contains a run of weight loading module and runs of all the feed module. In each iteration, the weight feeding module loads the weight tile into one of the half address space of weight BRAM buffers while the feed modules access the weight data tile from loaded in the previous iteration from the other half address and stream the data to PE array.  The dual-port architecture of BRAM enables the concurrent runs of the weight load module and the feed modules. We can observe that each row of the PE array requests weight data with one cycle delay than its previous row, as shown in Fig. \ref{fig:winosystolic}. We insert FIFOs with incrementing depth between the feed output port and PE array to accommodate the incrementing delay.\\
% \subsubsection{Plannal Input Data Access Subsystem}~\label{sect:weight_data_system}\\
% \fi






\subsection{Software Implementations}
% In order evaluate the efficiency of our Winograd convolution IP within a real CNN, 

\subsubsection{Layer allocation:}
In order to enable the end-to-end execution of any given CNN models,
we implement the non-convolution layers, such as element-wise addition, average/max pooling, fully connected, as software kernels that are executed on the processor cores of our target platform. 
The software kernels are written in C/C++ with posix threads to evenly allocate and parallelize the kernels across all available processor cores. As these kernels are typically memory bounded, we parallelize the work across output channel dimensions to minimize the sharing of dirty cache lines.

\subsubsection{Model compilation:}
The input model is first transformed and stored into a YAML\footnote{https://yaml.org/} file format. Then the host program turns the network model into a graph composed of feature-maps and layers.
The host program also allocates memory for each feature-map in the external memory (DDR) and schedules the layer execution based on the data dependency in topological order.
After the scheduling is determined, the host program calls either the software layer or the hardware layer as scheduled.
% \todo[inline]{Add in the link of 'how to use the hardware configuration information'.}




==> bak/sec8.tex <==

\section{System Modeling}\label{sec:modeling}

Since our proposed system is built based on performance and resource sensitive parameters,
manually finding their optimal values is time consuming.
Therefore, we build analytical resource and performance models of the design parameters to ease the design space exploration for our proposed system.

\subsection{Resource Model}
DSPs and BRAMs are the most critical resources in the FPGA platform, of which we mainly consider in our resource model. Although the LUT resource is also used as computing resources to construct adders in our design, it usually is not the bottleneck because of the good optimization of FPGA design tools and the light utilization of adders in our design.

\subsubsection{DSP estimation}
The major instances of DSPs used by the systolic WinoPE array. Each WinoPE needs to compute the element-wise sum of product along $Q$ input channels for $B$ transformed input tiles $U^{4\times4}$ and weight tiles $V^{4\times4}$. 
Each double-pumping DSP can complete the sum of products between 2 input channels. Thus, the total number of DSPs required by a WinoPE is $4\cdot 4\cdot B\cdot \lceil{Q/2} \rceil$. 
The systolic WinoPE array contains $M\times N$ WinoPEs, so the total DSP required in our WinoCNN accelerator can be computed as:
\begin{equation}
   DSP=16\cdot M\cdot N\cdot B\cdot \lceil{Q/2}\rceil 
\end{equation}


\subsubsection{BRAM estimation}
The BRAM resource is mainly occupied by the input, weight and output buffers. The Block RAM in the FPGA chip is organized as 18K-blocks, each is of 18-bit width and 1024 depth.
As shown by many previous works, weight data could be quantized to lower bitwidth without sacrificing the DNN model accuracy~\cite{ul2q, vecq}. In our design, in order to support a wide range of quantization methods and preserve the model accuracy, we support up to 7 bits of data width for the weights. After transformation, the bit-width of weight buffer is raised to 11 bit.

For weight buffer, each row of the systolic WinoPE array requires $4\cdot 4\cdot Q$ transformed weight data streamed in and thus requires $\lceil{4\cdot4\cdot Q\cdot 11/18}\rceil$ BRAM blocks to provide enough data access bandwidth. The total BRAM required for weight buffer is $M\cdot \lceil{ Q\cdot 176/18}\rceil$.

For output buffer, each WinoPE has a $4\times4$ buffer matrix which stores 8 bit output data of batch $B$. Each WinoPE requires 2 buffers for ping-pong access. Therefore, each WinoPE needs $2\cdot \lceil{16\cdot B\cdot 8/18}\rceil$ BRAMs as output buffer, and the whole WinoCNN accelerator needs $2\cdot M\cdot N\lceil{16\cdot B\cdot 8/18}\rceil$ BRAMs.

The input buffer, as discussed in Section \ref{sect:data_opt}, is a buffer matrix of size $H_b \times W_b$. Each bank should be capable of storing $B$ input data (8 bit). So the total BRAM data for the input is $H_b \cdot W_b \cdot \lceil{8\cdot B/18}\rceil$.

The total number of BRAMs can be calculated as:
%\vspace{-4pt}
\begin{equation}
\begin{gathered}
    BRAM=M\cdot \lceil{ Q\cdot 176/18}\rceil
    +2\cdot M\cdot N\lceil{ B\cdot 256/18}\rceil\\
    + H_b \cdot W_b \cdot \lceil{8\cdot B/18}\rceil\\
\end{gathered}
\end{equation}






\subsection{Latency Model}
% \textcolor{blue}{We design our Winograd systolic array based on the principle of configurability propose a latency model base on hardware parameters.}
% Our design maintains the following hardware parameters that could be configured: Winograd cell type (lite or combine),  PE array height $M$, PE array width $N$. 
% Also, we enable the input depth wise parallelism in the PE architecture with a configurable parallelism factor $Q$ and image batch size $B$. Meanwhile, a configurable constraint which is the communication bandwidth is denoted as $BW$. 

% According to Algorithm. \ref{alg:conv_schedule}, we can conclude the overall 
In our design, the latency of a convolution task is split into three parts: pre-loop input reading, computation loop and post-loop data offloading, denoted as $t_{pre}$, $t_{loop}$ and $t_{post}$, respectively.
The total latency is calculated as the sum of the three parts:
\vspace{-4pt}
\begin{equation}
    t_{total}= t_{pre} + t_{loop} + t_{post}
\end{equation}

To obtain an accurate latency modeling, we consider both the communication latency $t_{comm}$ and computation latency $t_{comp}$ in each phase of the convolution procedure,
whose latency is the maximum value among $t_{comm}$ and $t_{comp}$. The communication latency $t_{comm}$ is estimated as:
% \vspace{-4pt}
\begin{equation}
    t_{comm}=\frac{D_{total}}{BW}
\end{equation}
where $D_{total}$ is the total amount of data required to be transferred. 
The computation latency $t_{comp}$ differs based on the hardware architecture and internal scheduling of the computation kernel.

For pre-loop input reading and post-loop data output phase, the latency is restricted purely by the communication data rate and the total amount of the data,
which are the number of pixels read in or written out that are related to convolution configurations and row-step $RS$. Thus, we have the following estimations for $t_{pre}$ and $t_{post}$:
\begin{equation}
    t_{pre}=\frac{(RS+K-P)\cdot ID \cdot IW \cdot B}{BW}
\end{equation}
\begin{equation}
    t_{post}=\frac{RS\cdot OD \cdot OW \cdot B}{BW}
\end{equation}

For computation loop iterations, WinoCNN needs both off-chip data communication and computation.  
All the weights are required once within each loop iteration, thus we have $D_{weight}=F^2\cdot ID\cdot OD$ 
Meanwhile, each loop iteration in Algorithm \ref{alg:conv_schedule} includes a read input process and a write output process with corresponding data transmission amount as $D_{input}=RS\cdot ID \cdot IW \cdot B$ and $D_{output}=RS\cdot OD \cdot OW \cdot B$.
Neglecting the absence of write output process in the first iteration and the read input process in the last iteration, we estimate the communication latency as:
\begin{equation}
    t_{comm}=\frac{D_{weight}+D_{input}+D_{output}}{BW}
\end{equation}

The computation latency is decided by the configuration of WinoPE array. To compute $RS$ rows of outputs in each computation process, the WinoPE array needs to sum up the convolution results through $ID$ input planes to generate $RS\times OW$ output data for $OD$ output planes. In each cycle, $M\times N$ WinoPE sum up the convolution results of $Q$ input planes for $N\times K\times K$ output pixels along $M$ depth. Assuming the convolution system runs at a frequency $f$, the computation latency for each iteration could be calculated as:
\begin{equation}
    t_{comp}= \frac{1}{f} \cdot \left  \lceil{\frac{ID}{Q}}\right \rceil  
    \left\lceil{\frac{OD}{M}}\right \rceil
    \left\lceil{\frac{RS}{K}}\right \rceil
    \left\lceil{\frac{OW}{N\cdot K}}\right \rceil
\end{equation}
Since the communication and computation is pipelined, the latency for each loop iteration $t_{iter} = max(t_{comm},t_{comp})$ and consequently we have the latency for the computation loop as:

% \vspace{-4pt}
\begin{equation}
t_{loop} = \lceil{\frac{OH}{RS}} \rceil \cdot t_{iter}
\end{equation}
% Summarizing the pre-loop input reading, computation loop and post-loop outputting latency, we have the final latency model as:
% \todo[inline]{What is software combination? Also, I feel we are not well linking the equations above to the resource and performance, am I missing anything?}
% \todo[inline]{I need to add the resource estimation, the resource estimation is related to M,N,B,Q}
